Nonlinear Projection Based Gradient Estimation for Query Efficient Blackbox Attacks

Gradient estimation and vector space projection have been studied as two distinct topics. We aim to bridge the gap between the two by investigating how to efficiently estimate gradient based on a projected low-dimensional space. We first provide lower and upper bounds for gradient estimation under both linear and nonlinear projections, and outline checkable sufficient conditions under which one is better than the other. Moreover, we analyze the query complexity for the projection-based gradient estimation and present a sufficient condition for query-efficient estimators. Built upon our theoretic analysis, we propose a novel query-efficient Nonlinear Gradient Projection-based Boundary Blackbox Attack (NonLinear-BA). We conduct extensive experiments on four image datasets: ImageNet, CelebA, CIFAR-10, and MNIST, and show the superiority of the proposed methods compared with the state-of-the-art baselines. In particular, we show that the projection-based boundary blackbox attacks are able to achieve much smaller magnitude of perturbations with 100% attack success rate based on efficient queries. Both linear and nonlinear projections demonstrate their advantages under different conditions. We also evaluate NonLinear-BA against the commercial online API MEGVII Face++, and demonstrate the high blackbox attack performance both quantitatively and qualitatively. The code is publicly available at https://github.com/AI-secure/NonLinear-BA.

==> def.tex <==

\section{Problem Definition}
\bo{need to define blackbox attack etc, otherwise the following definitions read irrelevant }
\Huichen{how about this? (definition 2)}
We follow the convention of previous blackbox attack works and consider an attacker that can only access via queries a $C$-way classification machine learning model. 
\begin{definition}[Classification Model]
    The classification model is defined as a function $G:\,\bbR^m \mapsto \bbR^C$.
    The output of $G$ is the confidence score for each class.
    The model predicts the class $y = \argmax_{i\in [C]} G(x)_i$, i.e., the class with highest confidence score.
    \label{def:classification-model}
\end{definition}
% $y = \argmax_{i\in [C]}{G(x)_i}, x\in \mathbb{R}^m, G(x)\in \mathbb{R}^k$. 
\bo{may not need a definition here and need to define x y -- certain distribution}
\begin{definition}[Boundary-based Blackbox Attack]
The model's structure and parameter weights are assumed to be unknown to the attacker. The attacker has only `query' access to the model that inputs an image $x$ to the model and gets a label $y$ as the model prediction.
Suppose there is a \targetimage ${x}_{tgt} \in \bbR^m$ whose true label is $y_{ben} \in [C]$. The attacker's goal is to craft an \advimage ${x}_{adv}$ that is predicted as a maliciously chosen label $y_{mal} \in [C]$, while the distance $D({x}_{tgt}, {x}_{adv})$ between the two images is as small as possible. Here $D$ is a distance metric like $L_2$-norm distance or $L_\infty$-norm distance that 
%helps to 
restrict the perturbation added on the \targetimage in order to escape human notice.
    \label{def:black-box-attack}
\end{definition}
In this paper we only consider targeted attack with an intentionally chosen $y_{mal}$ since untargeted attack is a trivial extension of the targeted case (by randomly sampling a $y_{mal}$).
% 

For convenience, we define difference function $S$, which is the difference of prediction score for the malicious label $y_{mal}$ and for the true label $y_{ben}$.
Due to the blackbox setting, for any $x$, we can only query the sign of $S(x)$, i.e., $\sgn\left(S(x)\right)$.
\begin{definition}[Targeted Difference Function]
    Given model $G$, the target function $S:\,\bbR^m \to \bbR$ is defined by $S(x) = G(x)_{y_{mal}} - G(x)_{y_{ben}}$, where $y_{mal}$ is the adversarial target.
    \label{def:difference-function}
\end{definition}

In order to do the attack, the attacker starts with a \sourceimage ${x}_{src}$ sampled from the class with label $y_{mal}$, then moves the image towards the \targetimage ${x}_{tgt}$ by adding pixel-level perturbations while the attacker makes sure the perturbed image is always predicted as $y_{mal}$ thus the attack is valid.
For simplicity of later descriptions, images that lie on the decision boundary between $y_{ben}$ and $y_{mal}$ and is classified as $y_{mal}$ are called \emph{\boundaryimage}.

\begin{definition}[Boundary Image]
    The image $x$ is called a \emph{boundary image} if and only if $G(x)_{y_{mal}} = G(x)_{y_{ben}}$, i.e., $S(x) = 0$.
\end{definition}



==> method.tex <==
\section{Proposed Method}
\bo{what does pipeline mean?} \Huichen{how about `proposed method' then?}
We first introduce the overall blackbox boundary-based attack pipeline
% which is an extension of 
% % the 
% QEBA~\cite{cvpr2020QEBA} 
% % paper
% . 
\Linyi{Delete ``is an extension of QEBA'', since it is confusing by mentioning both QEBA and HSJA.}
Given a victim machine learning model $G$, a \targetimage and a \sourceimage, the iterative algorithm for updating the adversarial image consists of three main step following 
% the 
HSJA~\cite{chen2020hopskipjumpattack}
% work~\Huichen{cite HSJA}
: 
(1)~estimate gradient at $G$'s decision boundary, (2)~move the image along estimated gradient direction, and (3)~map back to the decision boundary. 
Each step is done by querying the model with crafted input images and analysing the output labels. 
Typically, the first step is the most costly in terms of query numbers, taking about $100$ steps per iteration. The second and third steps take about $2$ to $6$ steps each, depending on the precision required in the step size search and the error tolerance during the binary search for decision boundary.
\Linyi{step or query?}

\paragraph{Estimate gradient at $G$'s decision boundary.}
In the original HSJA paper, the gradient estimation is done by Monte Carlo sampling method:
\begin{align}
    \widetilde{\nablaS(\xadv{t})} = \frac1B \sum_{b=1}^B \sgn \left(S\left(\xadv{t}+\delta {u}_b\right) \right) { u}_b,
    \label{eq:MC_gradient_estimation}
\end{align}

% \begin{align}
%     \widetilde{\nablaS(\xadv{t})} = \nabla f(0)^\T \cdot \left( \frac1B \sum_{i=1}^B \sgn \left( S \left( \xadv{t} + f(\delta * v_b) - f(0) \right) \right) v_b \right)
% \end{align}

where $\xadv{t}$ is the \boundaryimage at iteration $t$, ${ u}_b$'s are $B$ normalized perturbation vectors sampled from the whole gradient space. 
% The function $\phi(x)$ is an indicator function indicating whether the input is predicted as the target label $y_{mal}$ or not. 
The function $\sgn\left(S(\cdot)\right)$ is the sign of the difference function~(\cref{def:difference-function}).
% The value of the indicator function 
Its value is acquired by querying the victim model and compare the output label with $y_{mal}$.
The challenge is the high query cost when the input dimension $m$ is large. A typical $3$-channel $224\times 224$ image gradient vector has a dimension $m$ of over $150$k. It's very hard to perform accurate estimation in such a high-dimensional space with limited queries.
In order to reduce query complexity, QEBA proposes to find a `representative subspace' with orthonormal mappings $\bW=[w_1, \ldots, w_n] \in \mathbb{R}^{m\times n}, n \ll m$ and $\bW^\intercal \bW = I$. The perturbation vectors are generated by first sampling $n$ dimensional normalized vectors ${ v}_b$ and project with ${ u}_b = \bW { v}_b$.

\Linyi{Mention what is $\delta$?}

\paragraph{NonLinear-BA: estimation with nonlinear projection.}
\Linyi{Add a paragraph title to address our contribution.}
We generalize the gradient estimation with nonlinear projection. 
A good choice for the projection functions are machine learning generative models. We propose three choices for them: Auto-encoders (AE), Variational Auto-encoders (VAE) and Generative Adversarial Networks (GAN). Note that all these models typically have two components: an `encoder' and a `decoder' for AE and VAE, and a `generator' and a `discriminator' for the GANs. 
The `decoder' or `generator' projects a latent representation or random vector to sample space. The latent dimension is usually much lower than the sample space in this projection and this property is exactly desired. We unify the notations and denote both the `decoder' part of AE and VAE and the `generator' part of GAN as `projector' in our discussion. 

There are two phases of a blackbox boundary-based attack: training and attacking. 
During the training phase, the attacker first train a set of reference models on their own for the chosen dataset. The reference models are generally assumed to have different structure compared with the blackbox victim model. 
Then the generative models are trained on ground truth gradient images generated by the reference models. The `decoder' or `generator' part of the generated model is then used as the projector in the attacking phase. 
The detailed model structure and training settings will be described at Section~\ref{sec:exp}. Once the projector $\f:\bbR^n \to \bbR^m$ is trained, we first randomly sample normalized latent vectors ${ v}_b$'s. Then the perturbation vectors are generated as ${ u}_b = \f({ v}_b)$ and are used in the gradient estimation formula~\ref{eq:MC_gradient_estimation},
which yields our gradient estimator
\begin{equation}
    \widetilde{\nablaS(\xadv{t})} = \frac1B \sum_{b=1}^B \sgn \left(S\left(\xadv{t}+\delta \f({v}_b)\right) \right) \f({v}_b).
    \label{eq:our_gradient_estimation}
\end{equation}

\paragraph{Move the image along estimated gradient direction.}
After getting the estimated gradient $\widetilde{\nabla S}$, the \boundaryimage $\xadv{t}$ is moved along that direction by:
\begin{align}
    \label{eqn:move-grad}
    \hat{ x}_{t+1} = \xadv{t} + \xi_t \cdot \frac{\widetilde{\nabla S}}{\|\widetilde{\nabla S}\|_2}
\end{align}
where $\xi_t$ is a step size chosen by searching with queries following HSJA~\cite{chen2020hopskipjumpattack}.%\Huichen{cite}.

\paragraph{Map back to the decision boundary. }
In order to move closer to the \targetimage and enable the gradient estimation in the next iteration, we need to map the new adversarial image $\xadv{t}$ back to the decision boundary. This is achieved via binary search with the assistance of queries to find a suitable weight $\alpha_t$:
\begin{align}
    \label{eqn:binary}
    \xadv{t+1} = \alpha_t \cdot { x}_{tgt} + (1-\alpha_t) \cdot \hat{ x}_{t+1}.
\end{align}

